Smoothed Analysis with Adaptive Adversaries

We prove novel algorithmic guarantees for several online problems in the smoothed analysis model. In this model, at each time an adversary chooses an input distribution with density function bounded above by $\tfrac{1}{\sigma}$ times that of the uniform distribution; nature then samples an input from this distribution. Crucially, our results hold for {\em adaptive} adversaries that can choose an input distribution based on the decisions of the algorithm and the realizations of the inputs in the previous time steps. This paper presents a general technique for proving smoothed algorithmic guarantees against adaptive adversaries, in effect reducing the setting of adaptive adversaries to the simpler case of oblivious adversaries. We apply this technique to prove strong smoothed guarantees for three problems: -Online learning: We consider the online prediction problem, where instances are generated from an adaptive sequence of $\sigma$-smooth distributions and the hypothesis class has VC dimension $d$. We bound the regret by $\tilde{O}\big(\sqrt{T d\ln(1/\sigma)} + d\sqrt{\ln(T/\sigma)}\big)$. This answers open questions of [RST11,Hag18]. -Online discrepancy minimization: We consider the online Koml\'os problem, where the input is generated from an adaptive sequence of $\sigma$-smooth and isotropic distributions on the $\ell_2$ unit ball. We bound the $\ell_\infty$ norm of the discrepancy vector by $\tilde{O}\big(\ln^2\!\big( \frac{nT}{\sigma}\big) \big)$. -Dispersion in online optimization: We consider online optimization of piecewise Lipschitz functions where functions with $\ell$ discontinuities are chosen by a smoothed adaptive adversary and show that the resulting sequence is $\big( {\sigma}/{\sqrt{T\ell}}, \tilde O\big(\sqrt{T\ell} \big)\big)$-dispersed. This matches the parameters of [BDV18] for oblivious adversaries, up to log factors.

==> Algorithms.tex <==
    
    Note that the statistical bound on the regret in the previous section also comes with an algorithm. 
    Unfortunately, this algorithm is not efficient since it involves constructing a net over the class of hypotheses. 
    We would like to construct hypothesis classes that have efficient running times 
    
    In this section, we will construct algorithms the get sublinear regret against smoothed adaptive adversaries. 
    The idea is adapt the standard FTPL algorithm to the smoothed setting. 

    

FTPL



==> anti-concentration.tex <==
\paragraph{Our approach: a coupling based reduction.}
We introduce a general technique for reducing smoothed analysis with adaptive adversaries to to smoothed analysis of oblivious adversaries. 
Our technique is
based on a \emph{coupling} argument, that is a joint distribution connecting, $T$ random variables $(X_1, \dots, \X_T)$ that are generated by an adaptive smooth adversary  with $kT$ random variables $Z_i^{(t)}$ for $i\in [k]$ and $t\in [T]$ that are generated i.i.d.~from the uniform distribution.
A key aspect of this coupling is a monotonicity property, that when $k = \tilde{O}(1/\sigma)$ with high probability, 
     $ \left\{ X_1 , \dots , X_t\right\} \subseteq \big\{ Z_i^{\left( j \right)} \mid i \in \left[ k \right] , j\in \left[ t \right] \big\}$. 


This coupling demonstrate structural properties that are ideal for preserving and analyzing anti-concentration properties of smooth adversaries.
This monotonicity property paired with the fact that $Z_i^{(t)}$ are i.i.d~uniform variables are 
especially useful for using algorithms and proof techniques from the oblivious world that rely on anti-concentration and adapting them to work with adaptive adversaries.
That is, if an algorithm's failure mode is only triggered when $X_1 , \dots , X_t$ concentrate,
then replacing in $\big\{ Z_i^{\left( j \right)} \mid i \in [k] , j\in [t] \big\} \supseteq  \{X_1 , \dots , X_t\}$ only increase the likelihood of hitting the failure mode.
On the other hand, i.i.d.~uniform random variables $Z_i^{(t)}$s demonstrate excellent  anti-concentration properties and existing smoothed and average case analysis technique are designed to leverage these anti-concentration properties to achieve improved performance compared to the worst-case. 

We show the versatility of this simple coupling technique by considering problems from online learning, online discrepancy, and dispersion in online optimization. In each of these problems, we identify the anti-concentration property that previous work have used to deal with oblivious stochastic and smooth adversaries. In the case of online learning, this is anti-concentration of the input instances in  the symmetric difference between a hypothesis class and  its finite cover. In the case of online discrepancy, this is anti-concentration of correlations discrepency vectors and inputs. In the case of dispersion, this is anti-concentration of function discontinuities in small intervals.
Once these properties are identified, the coupling argument lifts them to hold for adaptive sequences through.  



\subsection{Anti-concentration Paragraphs }


In most applications where smoothed or average case analysis have led to drastic improvement over the worst-case analysis, algorithm design or analysis is leveraging anti-concentration properties of the input to get these improvements. 
However, as the process of creating an input becomes more and more adaptive, that is, as the adversary correlates the distribution of its current instances with the realizations of earlier instances and algorithm's actions, 
the randomness and anti-concentration properties of the input or the state of the algorithm may weaken.
Additionally,  correlations between future and past instances also create challenges as many of the tools that are used in smoothed analysis rely on the independence of input. 
Our coupling approach implicitly shows that adaptivity in smoothed analysis does not significantly weaken the anti-concentration properties of the input and allow us to lift algorithmic ideas and analysis that are designed for oblivious or stochastic adversaries to design and analyze algorithms that interact with an adaptive smooth adversary.


An important property of our coupling is that, with high probability, $\left\{ X_1 , \dots , X_t\right\} \subseteq \big\{ Z_i^{\left( j \right)} \mid i \in [k] , j\in [t] \big\}$.
This set containment property along with the fact that $Z_i^{(t)}$ are i.i.d uniform variables is an especially useful feature for lifting algorithms and proof techniques from the oblivious world that rely on anti-concentration. That is, when algorithm's failure mode is only triggered by the concentration of $X_1 , \dots , X_t$, then replacing in $\big\{ Z_i^{\left( j \right)} \mid i \in [k] , j\in [t] \big\} \supseteq X_1 , \dots , X_t$ can only increase the likelihood of hitting a failure mode.
On the other hand, uniform and independent random variables, $Z_i^{(t)}$s, demonstrate excellent  anti-concentration properties that are superior to most other offline stochastic or oblivious smooth distributions.  Therefore, existing proofs and algorithms that work well in the stochastic or oblivious smooth settings, will continue to work well for adaptive smooth adversaries. 



==> app_coupling_proofs.tex <==
\section{Proofs from }

==> discrepancy_ALS.tex <==
    In this section, we will talk about a smoothed version of the online vector balancing problem. 
    The aim is find a sign $\epsilon_i$ upon seeing vector $v_i$ with $\norm{v_i} \leq 1 $ such that 
    \begin{equation*}
        \norm{ \sum_{i = 1}^t \epsilon_i v_i }_{\infty}
    \end{equation*}
    is small for each $t \leq T$. 
    The problem can be generalized to other choices of norms but we will restrict the discussion to the infinity norm. 
    Note that choice of sign at time $t$ can only be function of the vectors up to time $t$ and the norm of the vector must be small for all times.  
    In the fully adversarial model, where the choice of the vector $v_t$ could depend on the past choice of signs of the algorithm, the only a trivial $O\left( \sqrt{T} \right)$ bound can be achieved. 
    Thus, it is interesting to consider relaxed semi-random models of the adversary such that we can recover non-trivial bounds. 

    We work in the setting where $v_i$ are generated from a $\sigma$-smooth distribution which is adpatively chosen after the choice of $\epsilon_1 \dots \epsilon_{t-1}$ has been made. 
    This choice interpolates between a fully stochastic adversary and a fully adaptive adversary. 
    In this section, we give discrepancy bounds that smoothly interpolate between the stochastic and adaptive cases.  

        


    \begin{theorem}
        Let $\adist_i$ be an adaptive sequence of distributions $\sigma$-smooth distributions such that $X_i \sim \adist_i$. 
        There is an algorithm that produces signs $\epsilon_i$ such that 
        \begin{equation*}
            \norm{ \sum_{i = 1}^t \epsilon_i X_i   } \leq O\left( \log\left( \frac{20 T n \log \left( \frac{10 T}{\delta} \right)  }{\sigma \delta} \right) \right) 
        \end{equation*}
        for all $t\leq T$ with probability $1 - \delta$. 
    \end{theorem}
    \begin{proof}
        Let $\epsilon_i$ denote the signs to be assigned to $X_i$. 
        We inductively construct the signs using the algorithmic ideas from \cite{ALS_Disc}. 
        Let $\epsilon_1 \dots \epsilon_{t-1}$ be fixed already.
        We will see how to construct $\epsilon_t$.  
        Let $ \adist_t \left( X_ 1, \dots, X_{t-1} , \epsilon_1 , \dots , \epsilon_{t-1} \right) $ be the smooth distribution of the adversary at time $t$ and let $ X_t \sim \adist_t \left( X_ 1, \dots, X_{t-1} , \epsilon_1 , \dots , \epsilon_{t-1} \right) $
        The idea is to use the algorithm from \cite{ALS_Disc} to find a signing for $X_t$. 
        Also, let $w_{t-1} = \sum_{i=1}^{t-1} \epsilon_i X_i   $ be the discrepancy vector till time $t-1$ and let $c$ be a threshold that we will decide later. 
        If $\norm{w_{t-1}}_{\infty} \geq c  $ or if  $\abs{ \ip{w_{t-1}}{ X_t } }  > c$, we declare failure. 
        Else, let 
        \begin{equation*}
            \epsilon_t = \begin{cases}
                1 & \text{with probability } \frac{1}{2} - \frac{ \ip{w_{t-1}}{ X_t } }{2c} \\
                - 1 & \text{with probability } \frac{1}{2} + \frac{ \ip{w_{t-1}}{ X_t } }{2c} 
            \end{cases}
        \end{equation*}
        be the sign at time $t$. 
        As in \cite{ALS_Disc}, define $\mathcal{B}_t \left( X_1 , \dots , X_t \right)  $ to be the following distribution
        \begin{itemize}
            \item If $\abs{\ip{w_i}{ X_{i+1} } } > c   $ or $  \norm{w_i}_{\infty} > c $ for some $i$, then all the mass is on zero. Let us denote this as the bad event.
            \item Else, corresponds to the distribution of $w_t$.   
        \end{itemize}
        We want to show that for all time $ t $, $ \tilde{w}_{t-1}  \sim \mathcal{B}_{t-1} $, $ \abs{\ip{ \tilde{w}_{t-1} }{X_t } } < c   $ and $ \norm{\tilde{w }_{t}  }_{\infty} \leq c $ with probability greater than $\delta$.  
        Working inductively, it suffices to bound the additional mass that $\mathcal{B}_t $ puts on the bad event. 
        This can be bounded by bounding the probability that 
        \begin{equation*}
            \Pr_{ \tilde{w}_{t - 1} \sim \mathcal{B}_{t - 1} , X_t \sim \adist_t }  \left[ \abs{ \ip{\tilde{w}_{t - 1}}{ X_t } } > c \right] 
        \end{equation*}
        and 
        \begin{equation*}
            \Pr_{ \tilde{w}_{t } \sim \mathcal{B}_{t } } \left[ \norm{\tilde{ w}_t  }_{\infty} > c \right] .
        \end{equation*}
        This suffices since all the mass of the bad event is moved to zero. 

        We will show that this algorithm produces a sequence of signings with good discrepancy using ideas from the coupling argument from \cref{sec:main_coupling}. 
        From \cref{lem:single_round}, we have a coupling $\Pi_t$ on $\left( \tilde{X_t} , Z_1^{\left( t \right)} , \dots , Z_k^{\left( t \right)} \right)$ such that $\tilde{X_t}$ is distributed according to $\adist_t \left( X_ 1, \dots, X_{t-1} , \epsilon_1 , \dots , \epsilon_{t-1} \right)$ and $ Z_1^{\left( t \right)} , \dots , Z_k^{\left( t \right)} $ are independent and uniformly distributed. 
        Now, let us consider the $k$ copies of the step $t$ of the algorithm, one each corresponding to $Z_i^{\left( t \right)}$. 
         That is, we declare failure if  $\abs{ \ip{w_{t-1}}{ Z_i^{\left( t \right)} }   }  > c$ or else
         \begin{equation*}
            \epsilon^{i}_t = \begin{cases}
                1 & \text{with probability } \frac{1}{2} - \frac{ \ip{w_{t-1}}{ Z_i^{\left( t \right)} } }{2c} \\
                - 1 & \text{with probability } \frac{1}{2} + \frac{ \ip{w_{t-1}}{ Z_i^{\left( t \right)}   } }{2c} 
            \end{cases}
        \end{equation*} 
        Note that from \cref{lem:single_round} under $\Pi_t$ with probability at most $ \left( 1 - \sigma \right)^{k} $, we have that $ \tilde{X_t} \notin \left\{  Z_1^{\left( t \right)} , \dots , Z_k^{\left( t \right)} \right\} $. 
        Let us denote this failure event by $\mathcal{E}_t$.
        Now, note that 
        \begin{equation*}
            \Pr_{ \tilde{w}_{t - 1} \sim \mathcal{B}_{t - 1} , X_t \sim \adist_t }  \left[ \abs{ \ip{\tilde{w}_{t - 1}}{ X_t } } > c \right] = \Pr_{\Pi, \tilde{w}_{t - 1} \sim \mathcal{B}_{t - 1} } \left[ \abs{ \ip{\tilde{w}_{t - 1}}{ \tilde{X}_t } } > c \right]
        \end{equation*}
        since $\tilde{X}_t $ has the same distribution as $ X_t $. 
        \begin{align*}
            \Pr_{\Pi, \tilde{w}_{t - 1} \sim \mathcal{B}_{t - 1} } \left[ \abs{ \ip{\tilde{w}_{t - 1}}{ \tilde{X}_t } } > c \right] &= \Pr_{\Pi, \tilde{w}_{t - 1} \sim \mathcal{B}_{t - 1} } \left[ \mathcal{E}_t \land  \abs{ \ip{\tilde{w}_{t - 1}}{ \tilde{X}_t } } > c \right] + \Pr_{\Pi, \tilde{w}_{t - 1} \sim \mathcal{B}_{t - 1} } \left[  \overline{ \mathcal{E}_t} \land \abs{ \ip{\tilde{w}_{t - 1}}{ \tilde{X}_t } } > c \right] \\ 
            & \leq  \Pr \left[ \mathcal{E }_t  \right] + \Pr_{\Pi, \tilde{w}_{t - 1} \sim \mathcal{B}_{t - 1} } \left[  \overline{ \mathcal{E}_t} \land \abs{ \ip{\tilde{w}_{t - 1}}{ \tilde{X}_t } } > c \right] \\ 
            & \leq \left( 1 - \sigma \right)^{k} + \Pr_{\Pi, \tilde{w}_{t - 1} \sim \mathcal{B}_{t - 1} } \left[  \overline{ \mathcal{E}_t} \land \abs{ \ip{\tilde{w}_{t - 1}}{ \tilde{X}_t } } > c \right] \\ 
            & \leq \left( 1 - \sigma \right)^{k} +  \Pr_{\Pi, \tilde{w}_{t - 1} \sim \mathcal{B}_{t - 1} } \left[  \overline{ \mathcal{E}_t} \land \exists j \in \left[ k \right] \abs{ \ip{\tilde{w}_{t - 1}}{ Z_{j}^{\left( t \right)}  } } > c \right] \\
            & \leq \left( 1 - \sigma \right)^{k} +  \Pr_{\Pi, \tilde{w}_{t - 1} \sim \mathcal{B}_{t - 1} } \left[  \exists j \in \left[ k \right] \abs{ \ip{\tilde{w}_{t - 1}}{ Z_{j}^{\left( t \right)}  } } > c \right] . 
        \end{align*}
        In order to bound the second term, we first use the union bound. 
        \begin{align*}
            \Pr_{\Pi, \tilde{w}_{t - 1} \sim \mathcal{B}_{t - 1} } \left[  \forall j \in \left[ k \right] \abs{ \ip{\tilde{w}_{t - 1}}{ Z_{j}^{\left( t \right)}  } } > c \right]  &\leq k \cdot \Pr_{\Pi, \tilde{w}_{t - 1} \sim \mathcal{B}_{t - 1} } \left[\,  \abs{ \ip{\tilde{w}_{t - 1}}{ Z_{j}^{\left( t \right)}  } } > c \right] \\ 
            & \leq k \cdot \Pr_{Z \sim \mathcal{U},  \tilde{w}_{t - 1} \sim \mathcal{B}_{t - 1} } \left[\,  \abs{ \ip{\tilde{w}_{t - 1}}{ Z  } } > c \right] 
        \end{align*}
        The last line follows from the fact that in the coupling $\Pi$, the $Z_i$ were all independent and uniformly distributed. 
        In particular they are also independent of $X_1 \dots X_{t-1}  $ and $ \epsilon_1 \dots \epsilon_{t-1}$. 
       Now we recall the main theorem from \cite{ALS_Disc}. 
        \begin{lemma} [\cite{ALS_Disc}]
            For any fixed vector $u$, 
            \begin{equation*}
                \Pr_{\tilde{w}_{t - 1} \sim \mathcal{B}_{t - 1}} \left[ \abs{ \ip{ \tilde{w}_{t - 1}  }{u } } > c \right] \leq \sqrt{2} e^{ - c / 8 \pi }. 
            \end{equation*}
        \end{lemma}
        Thus, plugging this back into the earlier equations, we get 
        \begin{equation*}
            \Pr_{ \tilde{w}_{t - 1} \sim \mathcal{B}_{t - 1} , X_t \sim \adist_t }  \left[ \abs{ \ip{\tilde{w}_{t - 1}}{ X_t } } > c \right] \leq  \sqrt{2}k e^{ - c / 8 \pi} +\left( 1 - \sigma \right)^{k}. 
        \end{equation*}
        Repeating this for each standard basis vector $e_i$, we get the bound
        \begin{equation*}
            \Pr_{ \tilde{w}_{t - 1} \sim \mathcal{B}_{t - 1} , X_t \sim \adist_t }  \left[ \norm{w_{t - 1} }_{\infty} > c \land \abs{ \ip{\tilde{w}_{t - 1}}{ X_t } } > c \right] \leq  \sqrt{2}kn e^{ - c / 8 \pi} +\left( 1 - \sigma \right)^{k}. 
        \end{equation*}
        Setting $c = 8 \pi \log \left( \frac{20knT}{\delta} \right)$, we get that this is bounded by $\delta$. 
    \end{proof}
          



==> intro.tex <==
\section{Introduction (old)}








Offline and online learnability are two of the most classical problems in
the theory of machine learning. The first considers scenarios where a learner attempts to learn
a highly accurate hypothesis on instances that are drawn i.i.d. from some fixed but unknown
distribution and the second considers online scenarios where the instances are generated by an adversary.
Offline and online learnability are characterized by two different notions of
complexity of the hypothesis space: the VC dimension and the Littlestone dimension
respectively. In many hypothesis classes, however, there is a large gap between these two notions of complexity, and as a result, there is a gap in our ability to learn in the offline and online settings.
For example, while the class of $1$-dimensional threshold functions has
a VC dimension of $1$ and can be learned in the offline i.i.d. setting with convergence rate of
$O(\sqrt{T})$, but the Littlestone dimension of this class is unbounded, and so learning it in the  online adversarial setting incurs $O(T)$ regret.
Is there a middle ground between the i.i.d. and adversarial
models that can lead to strong learnability results, like those achievable in the offline setting, but is still robust to the presence of an adversary? Smoothed analysis provides one approach to this question.

Let us first consider the standard online learning setup with an
instance space $\X$ and a set $\H$ of binary hypotheses each mapping
$\X$ to $\Y =\{+1,-1\}$.  Online learning is played over $T$ time
steps, where at each step the learner picks a prediction function from
a distribution
and the \emph{adaptive} adversary chooses a pair of $(x_t, y_t) \in \X\times \Y$. The regret of an algorithm
is the difference between the number of mistakes the algorithm makes
and that of the best fixed hypothesis in $\H$. The basic goal in
online learning is to obtain a regret of $o(T)$. 


We extend this  model to accommodate smoothed adversaries.  We say that a distribution $\D$ over instance-label pairs is
{\em $\sigma$-smooth} if its density function over the instance domain is pointwise bounded by at most $1/\sigma$ times that of the uniform distribution.  In the online learning setting this means that at step $t$, the adversary chooses an arbitrary $\sigma$-smooth distribution $\D_t$ from which $(x_t, y_t)\sim \D_t$ is drawn. 



\begin{equation*}
	 \sum_{t=1}^T \mathbb{I}  \left( \hat{y_t} \neq y_t \right) - \min_{h \in  \mathcal{H} } \mathbb{I}  \left( h \left( x_t \right) \neq y_t \right) 
\end{equation*}


We would like to get regret that is sublinear in $T$.
When $\alpha = 0$, that is the typical setting of online adversarial setting with no smoothing, 
it is well-known that $\mathbf{Regret} \in \tilde\Theta(\sqrt{T~\mathrm{LDim}(\F)})$, where $\mathrm{LDim}(\F)$ is the Littlestone Dimension of $\F$.
We show that for general $\alpha$, i.e., non-zero smoothing, 
$\mathbf{Regret} \in \tilde\Theta(\sqrt{T~\mathrm{VCDim}(\F) \ln(1/\alpha)})$, where $\mathrm{LDim}(\F)$.
That is smoothed online learning is possible if and only if offline learning is possible.

\begin{theorem}[Main Theorem, Informal]
	There is an algorithm that achieves sublinear regret against smoothed, adaptive adversaries when the hypothesis class is of bounded VC-Dimension. 
\end{theorem}

\subsection{Model}

Let us first consider the standard online learning setup with an
instance space $\X$ and a set $\H$ of binary hypotheses each mapping
$\X$ to $\Y =\{+1,-1\}$.  Online learning is played over $T$ time
steps, where at each step the learner picks a prediction function from
a distribution
and the \emph{adaptive} adversary chooses a pair of $(x_t, y_t) \in \X\times \Y$. The regret of an algorithm
is the difference between the number of mistakes the algorithm makes
and that of the best fixed hypothesis in $\H$. The basic goal in
online learning is to obtain a regret of $o(T)$. 

We extend this model to accommodate smoothed adversaries.  We
say that a distribution $\D$ over instance-label pairs is
{\em $\sigma$-smooth} if its density function over the instance domain is
pointwise bounded by at most $1/\sigma$ times that of the uniform
distribution.  In the online learning setting this means that at step
$t$, the adversary chooses an arbitrary $\sigma$-smooth distribution
$\D_t$ from which $(x_t, y_t)\sim \D_t$ is drawn. 

Why should smoothed analysis help in online learning?  Consider the
well-known lower bound for $1$-dimensional thresholds over
$\X = [0,1]$, in which the learner may as well perform binary search
and the adversary selects an instance within the uncertainty region of
the learner that causes a mistake.  While the learner's uncertainty
region is halved each time step, the worst-case adversary can use
ever-more precision to force the learner to make mistakes
indefinitely. On the other hand, a $\sigma$-smoothed adversary
effectively has bounded precision. That is, once the width of the
uncertainty region drops below $\sigma$, a smoothed adversary can no
longer guarantee that the chosen instance lands in this region.
Similarly for differential privacy, there is a $\sigma$-smooth
distribution that produces the same answers to the queries. Such a
distribution has no more than $\alpha$ probability over an interval of
width $\sigma\alpha$. So one can focus on computing the errors of the
$1/(\sigma\alpha)$ hypotheses with discreized thresholds and learn a
hypothesis of error at most $\alpha$.
Analogous observations have been made in prior works
(\cite{NIPS2011_4262}, \cite{Cohen-Addad},
\cite{Gupta_Roughgarden}), although only for very specific
settings (online learning of $1$-dimensional thresholds,
$1$-dimensional piecewise constant functions, and parameterized greedy
heuristics for the maximum weight independent set problem, respectively).
Our work is the first to demonstrate the breadth of the settings
in which fundamentally stronger learnability guarantees are possible
for smoothed adversaries than for worst-case adversaries.



	\subsection{Related Work}
	The study of online learning in the presence of a smoothed adversaries has received some attention recently. 
	Below we consider a few works in this direction. 

	Online learning 

	Connecting online learnability and offline learnability 

	Littlestone dimension has also been studied in model theory under the name $2$-rank. 
	It can be shown that any class that has infinite Littlestone dimension must contain thresholds. 
	It was recently shown that any class that can be privately learnt must have infinite Littlestone dimension \cite{private_PAC}. 

	Smoothed analysis in algorithms 
	
	\cite{Gupta_Roughgarden} considers the problem of application specific algorithm design. 
	They consider the task of selecting a algorithm of a set of algorithms as a learning task and apply techniques from PAC learning and online learning to the problem. 
	The part of their work most relevant to the current paper is the online learning aspect of it. 
	They show that for the maximum weight independent set problem, there are instances that lead to linear regret. 
	In order to circumvent this lower bound, they consider smoothed instances of the problem and show that this leads to inverse polynomial regret (in the size of the instance) albeit linear in the time horizon. 
	This serves as a motivation to consider online learning in the smoothed setting and sets up a framework in which regret bounds against smoothed adversaries in online learning can be applied. 

	\cite{NIPS20114262} considers the online learning problem when the action set of the adversaries is constrained. 
	One of the constraints that they explicitly consider is the setting of smoothed adversaries. 
	They show that the regret of a smoothed adversary can be bounded by an appropriately defined sequential Rademacher complexity. 
	They also instantiate their bound for the class of thresholds and show $O \left( \sqrt{T} \right)  $ regret, which can shown to be unachievable in the non-smoothed setting. 

	\cite{Cohen-Addad} considers the online optimization of piecewise constant functions over the interval $\left[ 0,1 \right]$. 
	The model they consider is that of a non-adaptive adversary that specifies smooth distributions from which to generate discontinuities of the piecewise constant functions. 
	They give an algorithm that gets $O \left( \sqrt{T} \right) $ regret and can be implemented efficiently. 

	\cite{Dispersion} introduces a notion called dispersion which gives a condition on an instance under which they show that online learning can be done efficiently. 
	Roughly speaking, an instance of satisfies the dispersion condition if each ball of sufficiently small radius intersects the discontinuities of only a few of the functions. 
	They show that under the dispersion condition, they show guarantees from online learning and private batch optimization. 
	The paper also shows that non-adaptive adversaries drawing from a smooth distribution satisfies the dispersion condition. 

	The main difference between our work and the previous work is that we consider adaptive adversaries. 
	Previous work either shows regret bounds for specific classes \cite{NIPS20114262} or works under non-adaptive adversaries \cite{Cohen-Addad, Dispersion}. 
	Our analysis makes use of the sequential Rademacher complexity characterization of the minimax regret considered by \cite{NIPS20114262}. 
	 Our analysis also shows regret guarantees using the VC-dimension of a general class where as \cite{Dispersion} gives the bounds in terms of the dispersion. 
	It remains an interesting open question to prove or disprove that adaptive adversaries generate instances that are dispersed. 


	\subsection{Technical Challenges}
	In this section, we give a overview of the challenges and technical contributions of the paper. 
	We first summarize the techniques from the non-adaptive setting. 
	In this setting, the adversary decides a sequence of smooth distributions $\nadist_1, \dots \nadist_2$ ahead of time and points $x_1 \sim \nadist_1   \dots x_T \sim \nadist_T $ are samples from these distributions. 
	Note that here we have that each of the actions of the adversary is independent of the other. 
	That is, $x_i  $ and $x_j $ are statistically independent.  
	But, these are not all identically distributed and thus it is not immediately clear how to relate the error to statistical learning. 
	The idea is to consider a cover over the hypothesis class under the uniform distribution. 
	Since the distributions are smooth, this cover approximates the class even under the distributions of $\nadist_i$. 
	Since the samples are statistically independent, one can use ideas from uniform convergence to show that the difference in the classification error for the cover and classification error for the original hypothesis class is small.  
	Note that, since we are considering a cover under a fixed distribution, the size of the cover depends only on the VC-dimension of the class (and on the error parameter).
	 Since the cover is a finite set of hypotheses, one then can use a standard online learning algorithm, such as Hedge, in order to bound the regret.

	In the adaptive setting, the adversary can pick his distribution $\adist_i$ depending on the past instantiations of the noise. 
	Though, this difference does not lead to a issue in the non-smoothed setting, the difference is evident in the smoothed setting. 
	In particular, the previous proof idea does not carry over to this regime because the actions $x_j $ are no longer statistically independent and it is not clear how to apply ideas such as uniform convergence from statistical learning. 

	That said, we will still continue to work with the net.
	As before using a no-regret strategy on the net leads to the following decomposition of the regret. 
	\begin{equation*}
		\mathbb{E}[\regret(\A, \adist )] \leq  O\left( \sqrt{T \ln(|\H'|)} \right)  + \mathbb{E}_{\adist}\left[\max_{h\in \H}\min_{h'\in \H'} \sum_{t=1}^T 1\left(h(x_t) \neq h'(x_t) \right)  \right]. 
	\end{equation*}
	As noted before the issue is controlling the second term when the adversaries are adaptive. 
	For ease of notation, let us redefine this term as 
	\begin{equation*}
		\Ex_{\adist} \left[ \sup_{g \in \G } \sum_{i = 1}^T g\left( x_i \right)  \right] 
	\end{equation*}
	where  $\G = \{ g : \exists h \in \H \text{ and } h' \in \H' \text{ with } d\left( h , h' \right) \leq \epsilon \text{ and }  g = h \Delta h'  \}  $. 
	Thus, the problem reduces to a problem of bounding the maximum of a process index by a hypothesis class under distributions that do not have independence. 
	This will be our core technical challenge. 

	The main idea in this work is to construct a coupling between sequences of smooth distributions and the independent samples for the uniform distribution. 
	That is we construct a joint distribution between a sequence of random variables $X_1 \dots X_T$ and $Z_i^j$ such that the $X_i $ are distributed according to the smooth distribution of interest and the $Z_i^j$ are independent and uniformly distributed. 
	The main property that we want from the coupling is that the set $\left\{ X_1 \dots X_T\right\} $ is a subset of the set $ \left\{ Z_i^j \right\} $ with high probability. 
	The reason that this is interesting is that whenever we have $\left\{ X_1 \dots X_T\right\} \subset \left\{ Z_i^j \right\}  $, we have 
	\begin{equation*}
		\max_{g \in \G } \sum_{i = 1}^T g\left( X_i  \right) \leq \max_{g \in \G } \sum_{i,j} g\left( Z_{i}^j  \right) .
	\end{equation*}
	Thus, if this containment holds with sufficiently high probability, we can hope that the expectation is dominated by the expectation of the process on the right. 
	This is similar in idea to that of stochastic domination though there we would insist on a coupling such that term on the right would with probability one dominate the term on the left. 
	This difference turns out to be important as we shall discuss later. 

	In order to understand this coupling, let us look a simple example.
	Let the domain be the unit interval. 
	Consider a uniformly distributed random variable from the first half of the interval.
	This random variable is $ \nicefrac{1}{2} $ smooth. 
	Now, if we draw constantly many samples from the uniform distribution, we should expect at least one of them to be in the first half. 
	But conditioned on it being in the first half, we can think of this as being uniformly distributed on the first half. 
	This is the key idea behind the coupling that we construct. 
	This example already illustrates a technical consideration about the coupling allude to earlier in the discussion about stochastic domination. 
	Even though if we take sufficiently many samples from the uniform distribution we should expect at least one to be in a large set, we could get unlucky and have no sample in this set. 
	Thus, requiring the containment to always hold is a much more stringent requirement that ultimately will turn out to be unnecessary.  
	We extend this idea to general sequences of smooth distributions that are adaptive.   



	General ideas about couplings. 

	Coupling arguments are ubiquitous in probability theory. 
	They show up in many contexts such as when showing mixing, stochastic domination, optimal transport. 

	Coupling of point processes
	Stochastic domination



	




==> lower_bounds.tex <==
    \section{Lower Bounds}

    In this section, we first show that \cref{thm:regret-main} is tight up multiplicative $ \log  $ terms in $T$ and $ \log \log$ factors in $ \sigma  $ and $d$ and the additive $  d \sqrt{ \log\left(   \nicefrac{T}{d \sigma }  \right) } $ term. 
    In order to do this, we first formally define the notion of Littlestone dimension of a class.


    \begin{definition}[Littlestone Dimension, \cite{ben2009agnostic}]
        Let $\X$ be an instance space and $\F$ be a hypothesis class on $\X$. 
		A mistake tree is a full binary decision tree whose internal nodes are labelled by elements of $\X$. 
		For every choice of labels $ \{ y_i \}_{i=1}^d $, 
		Every root to leaf path in the mistake tree corresponds to a sequence $ \{  \left( x_i , y_i  \right) \}_{i=1}^{d}$ by associating a label $y_i$ to a node depending on whether it is the left or right child of its parent.   
		A mistake tree of depth $d$ is said to be shattered by a class $\F$ if for any root to leaf path $ \{  \left( x_i , y_i  \right) \}_{i=1}^{d}$, there is a function $f \in \F $ such that $ f\left( x_i \right) = y_i  $ for all $i \leq d$. 
		The Littlestone dimension of the class $\F$ denoted by $\lsd \left( \F \right) $ is the largest depth of a mistake tree shattered by the class $\F$. 
    \end{definition}

    The following theorem shows that the Littlestone dimension captures the regret in the online learning game against a class. 
    We will only need the lower bound but we will state the full theorem for completeness.   

    \begin{theorem}[\cite{ben2009agnostic,RegretTight}]\label{thm:regretLD}
        Let $\X$ be an instance space and $\F$ be a hypothesis class on $\X$. 
		Then, there exists an online learning algorithm $\mathcal{A}$ such that 
		\begin{equation*}
			\mathbf{Regret} \left( \mathcal{A} \right) \leq O\left(  \sqrt{   \lsd \left( \F \right) T  } \right).
		\end{equation*}
		Furthermore, for any algorithm $\mathcal{A}'$, we have that
		\begin{equation*}
			\mathbf{Regret} \left( \mathcal{A} '  \right) \geq \Omega \left(   \sqrt{  \lsd \left( \F \right) T  } \right) . 
		\end{equation*} 
    \end{theorem}

    Using the above theorem, we lower bound the regret in the online learning against smoothed adversaries. 
    We do this by reducing the smoothed case to the worst case for a related class and lower bound the worst case regret using the above theorem. 

    \begin{theorem}
        For every $d$ and $ \sigma $ such that $d \sigma\leq 1  $, there exists a $ \H $ such that for every algorithm there is an adversary such the regret is lower bounded by 
        \begin{equation*}
            \sqrt{dT \log \left( \frac{1}{\sigma d} \right) }. 
        \end{equation*}
    \end{theorem}
    \begin{proof}
        We will first construct a class on $\left[ \nicefrac{1}{\sigma} \right]$ with VC dimension $d$ and Littlestone dimension $ O\left( d \log \left( \nicefrac{1}{d \sigma} \right) \right) $. 
        For simplicity, assume $ \sigma^{-1}  $ and $ d $ to be powers of two. 
        Divide $ \left[ \nicefrac{1}{\sigma} \right] $ into $d $ subsets each of equal size, denoted by $A_i$. 
        On each of these subsets instantiate the class of thresholds i.e for each $\gamma \in A_i $, $ h_{\gamma} \left( x \right)  = 2\mathbb{I} \left[ x \geq \gamma \right] - 1 $ for $x \in A_i$ and $0 $ for $x \notin A_i$. 
        For a $d$-tuple of thresholds $ \left( h_{\gamma_1} \dots h_{\gamma_d} \right) $ with $\gamma_i \in A_i $, define the function 
        \begin{equation*}
            h_{ \gamma_1, \dots, \gamma_d  } \left( x \right) = \sum_{i=1}^d \mathbb{I} \left[ x \in A_i \right] h_{\gamma_i} \left( x \right). 
        \end{equation*} 
        This function can be seen as the union of the thresholds $h_{\gamma_i}$ thought of as subsets of the universe $\left[ \nicefrac{1}{\sigma} \right]$.  
        Define $\mathcal{H}$ to be the class of all such functions. 
        It is easy to see that this class has VC dimension $d$. 
        The VC dimension is at most $d$ since if any more than $d$ points would mean at least one of the $A_i$ must have two points but this cannot be shattered by thresholds on $A_i$. 
        The VC dimension can be seen to be at least $d$ by taking one point in each of the $A_i$.  

        We claim that this class has Littlestone dimension $ O\left( d \log \left( \nicefrac{1}{\sigma d} \right) \right) $. 
        In order to prove this associate to each string $ \left\{ -1, 1 \right\}^{d \log\left( 1 / \sigma d \right)} $ a function in $ \mathcal{H}$ as follows. 
        Divide the string into blocks of size $ \frac{1}{\sigma d}$. 
        We think of each of these blocks as forming a binary search tree for the subset $A_i$ by associating $ +1 $ to the right child of a node and $-1$ to the left child. 
        Thus, we path on this tree corresponds to a threshold by associating it with the threshold consistent with the labels along the path.  
        Doing this association separately for each block, we can associate the set of strings $ \left\{ -1, 1 \right\}^{d \log\left( 1 / \sigma d \right)} $ with a binary search tree with the leaves labeled by elements in $ \H$. 
        Also, note that this forms a fully shattered tree as required by the definition of the Littlestone dimension. 
        Thus, the Littlestone dimension of $ \H$ is $ d \log \left( \nicefrac{1}{\sigma d} \right) $. 
        
        Next consider the set $\left[ 0,1 \right]$ and divide it into contiguous subintervals of length $ \sigma $. 
        We define the projection function $ \Pi : \left[ 0,1 \right] \to \left[ \nicefrac{1}{\sigma} \right] $ by $ \Pi\left( x \right) = i  $ if $x$ is in the $i$th subinterval. 
        Define the class $ \G$ on $\left[ 0,1 \right] $ by composing $ \H $ with $ \Pi $ i.e. $ \G = \left\{  g : g = h \circ \Pi \right\} $. 
        Note that the uniform distribution on each subinterval is $ \sigma $-smooth. 
        Thus, in a smoothed online learning game with the class $\G $, an adversary who plays only uniform distributions on the subintervals defined above corresponds to an adversary in the usual online learning game on $ \left[ \nicefrac{1}{\sigma} \right] $ against class $\H$. 
        In particular, any algorithm for $\G$ against such an adversary can be converted to an algorithm for $\H$ with the same regret. 
        From \cref{thm:regretLD}, we have that the regret against $\H$ is lower bounded by 
        \begin{equation*}
            \sqrt{ T \ldim\left( \H \right) } = \sqrt{ dT \log\left( \nicefrac{1}{\sigma d} \right)  }
        \end{equation*}
        Thus, the regret in the smoothed online learning game for $\G$ is lower bounded by $ \sqrt{ dT \log\left( \nicefrac{1}{\sigma d} \right)  }$ as required. 
    \end{proof}


        




    Next, we show that the isotropy condition is required for the online discrepancy result.


    \begin{theorem}
        There is an adaptive sequence of $c\left( nT \right)^{-2} $-smooth (for some constant $c$) distributions on the unit ball such that for any online algorithm producing signs $\epsilon_i$,  we have 
        \begin{equation*}
            \norm{ \sum_{i=1}^T  \epsilon_i v_i }_{\infty} \geq \Omega \left( \sqrt{\frac{T}{n} } \right)
        \end{equation*}
        with probability $ 1 - e^{ - \frac{T}{12} } $. 
    \end{theorem}
    \begin{proof}
        To see the idea for the proof recall that without the smoothnes restriction, the adversary can pick vectors orthogonal to the discrepancy vector to induce high discrepancy. 
        We show that this can do essentially the same while maintaining some smoothness. 
        Let the discrepancy vector at time $t$ be denoted by $d_t$. 
        Consider the set $S_t = \left\{ x : \norm{x}_2 \leq 1, \abs{\ip{x}{ {d_{t-1}} } } \leq n^{-2} T^{-2} \norm{d_{t-1}}_2   \right\}$. 
        Note that the uniform distribution on $S_t$ is $ c n^{-2}T^{-2}  $ smooth for some constant $c$.  
        To see this, let $B$ be the unit ball and let $V_n$ denote the volume of the unit ball in $n$ dimensions. 
        Then, 
        \begin{align*}
            \Pr_{ X \sim B } \left[ X \in S_t \right] &= \frac{1}{V_n} \int_{-n^{-2}T^{-2} }^{n^{-2} T^{-2}} \left( 1 - x^2 \right)^{\frac{n-1}{2}} V_{n-1} dx \\ 
            & \geq \frac{1}{V_n} \int_{-n^{-2}T^{-2} }^{n^{-2} T^{-2}} \left( 1 - \frac{1}{n^4 T^4}  \right)^{\frac{n-1}{2}} V_{n-1} dx \\ 
            & \geq \frac{V_{n-1}}{V_n} \cdot  \frac{1}{ 2 n^{2}T^2 } \\ 
            & \geq \frac{1}{ 20 n^{2}T^2 }. 
        \end{align*}
        The second inequality follows by noting that $ \left( 1 - n^{-4}T^{-4} \right)^{\frac{n-1}{2}}  \geq \nicefrac{1}{4} $. 
        With this, we describe the adversary's strategy. 
        At time $t$, the adversary picks $v_t$ uniformly from $S_t$. 
        We will measure the squared $2$-norm of the discrepancy vector. 
        \begin{align*}
            \norm{d_{t}}^2_2 &= \norm{ \epsilon_t v_t + d_{t-1} }^2_2 \\ 
            & = \epsilon_t^2 \norm{v_t}^2_2 + \norm{d_{t-1}}^2_2 + 2 \ip{v_t}{d_t} \\ 
            & \geq \norm{v_t}^2_2 +   \norm{d_{t-1}}^2_2 - \frac{2 \norm{d_{t-1}}_2  }{n^2T^2} \\ 
            & \geq \norm{v_t}^2_2 +\norm{d_{t-1} }^2_2  - \frac{2}{ n^2 T } \\ 
            & \geq \sum_{i=1}^t \norm{v_i}_2^2  - \frac{2t}{n^2 T} . 
        \end{align*}
        Note that $ \Pr\left[ \norm{v_i} \leq \nicefrac{1}{2}  \right] \leq 2^{-\left( n-1 \right)} $. 
        This can be seen by noting that the probability can be computed with an integral similar to the one above but with ball of radius $\nicefrac{1}{2}$ instead of the ball of radius $1$.
        Also, note that $ \norm{v_i} $ are independent across $i$. 
         Denote $z_i$ as a random variable which $1$ if $ \norm{v_i} \geq \nicefrac{1}{2} $ and $0$ otherwise. 
         Then, 
        \begin{equation*}
             \sum_{i=1}^t \norm{v_i}_2^2 \geq \frac{1}{4} \sum_{i=1}^t z_i 
         \end{equation*}
        Applying a Chernoff bound to $z_i$, we get 
        \begin{equation*}
            \Pr\left[ \sum_{i=1}^t \norm{v_i}^2_2 \leq \frac{t}{8} \left( 1 - 2^{-\left( d-1 \right)  }\right) \right] \leq e^{ - \frac{  t  }{12} }. 
        \end{equation*}
        Thus with probability $1 - e^{- \frac{t}{12}}$, we have 
        \begin{equation*}
            \norm{d_t}^2_2 \geq \frac{t}{ 16} - \frac{2t}{n^2T } \geq \frac{t}{20}. 
        \end{equation*}
        We get the desired result by relating the $2$-norm and $\infty$-norm. 
    \end{proof}

    This shows that we cannot get the logarithmic dependence on smoothness parameter $\sigma $, $n$ and $T$ simultaneously without further assumptions on the distribution such as isotropy. 

==> macros.tex <==
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\renewcommand{\algorithmicensure}{\textbf{Output:}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}



\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}



\newcommand{\stringset}[1]{\{0,1\}^{#1}}
\newcommand{\bn}{\mathbb{N}}
\newcommand{\br}{\mathbb{R}}
\newcommand{\bz}{\mathbb{Z}}
\newcommand{\bq}{\mathbb{Q}}
\newcommand{\bc}{\mathbb{C}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\N}{\mathcal{N}}




\newcommand{\Z}{\mathcal{Z}}
\newcommand{\ip}[2]{\left\langle #1, #2 \right\rangle}

\newcommand{\Secref}[1]{\hyperref[#1]{Section \ref*{#1}}}
\newcommand{\Appref}[1]{\hyperref[#1]{Appendix \ref*{#1}}}

\DeclareMathOperator{\ent}{S}
\DeclareMathOperator*{\Ex}{\mathbb{E}}
\DeclareMathOperator{\tr}{\mathsf{tr}}
\DeclareMathOperator{\dt}{\mathsf{det}}
\DeclareMathOperator*{\argmin}{argmin}


\newcommand{\card}[1]{\lvert#1\rvert}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\bigSet}[1]{\bigl\{#1\bigr\}}
\newcommand{\BigSet}[1]{\Bigl\{#1\Bigr\}}
\newcommand{\braces}[1]{\{#1\}}
\newcommand{\Braces}[1]{\left\{#1\right\}}
\newcommand{\bigBraces}[1]{\bigl\{#1\bigr\}}
\newcommand{\BigBraces}[1]{\Bigl\{#1\Bigr\}}
\newcommand{\bracks}[1]{[#1]}
\newcommand{\bigBracks}[1]{\bigl[#1\bigr]}
\newcommand{\BigBracks}[1]{\Bigl[#1\Bigr]}
\newcommand{\biggBracks}[1]{\biggl[#1\biggr]}
\newcommand{\BiggBracks}[1]{\Biggl[#1\Biggr]}
\newcommand{\Bracks}[1]{\left[#1\right]}
\newcommand{\parens}[1]{(#1)}
\newcommand{\Parens}[1]{\left(#1\right)}
\newcommand{\bigParens}[1]{\bigl(#1\bigr)}
\newcommand{\BigParens}[1]{\Bigl(#1\Bigr)}
\newcommand{\biggParens}[1]{\biggl(#1\biggr)}
\newcommand{\BiggParens}[1]{\Biggl(#1\Biggr)}
\newcommand{\given}{\mathbin{\vert}}
\newcommand{\bigGiven}{\mathbin{\bigm\vert}}
\newcommand{\BigGiven}{\mathbin{\Bigm\vert}}
\newcommand{\biggGiven}{\mathbin{\biggm\vert}}
\newcommand{\bigNorm}[1]{\bigl\lVert#1\bigr\rVert}
\newcommand{\BigNorm}[1]{\Bigl\lVert#1\Bigr\rVert}
\newcommand{\Abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\BigAbs}[1]{\Bigl\lvert#1\Bigr\rvert}
\newcommand{\biggAbs}[1]{\biggl\lvert#1\biggr\rvert}
\newcommand{\angles}[1]{\langle#1\rangle}
\newcommand{\floors}[1]{\lfloor#1\rfloor}
\newcommand{\Floors}[1]{\left\l\floor#1\right\rfloor}
\newcommand{\Ceils}[1]{\left\lceil#1\right\rceil}
\mathchardef\dash="2D

\newcommand{\vcd}{\mathrm{VCDim}\xspace}
\newcommand{\lsd}{\mathrm{LDim}\xspace}
\newcommand{\regret}{\textsc{Regret}}


\newcommand{\combo}[3]{\Braces{#1}_{#2}^{#3}}
\newcommand{\red}[1]{{\color{red}#1}}
\addauthor{nh}{magenta}
\addauthor{as}{cyan}
\addauthor{tr}{blue}


==> prelim.tex <==
\section{Preliminaries}

Throughout this paper, we use $\X$ to denote an instance space and $\Y = \{0, 1\}$ to be the set of outcomes. A \emph{hypothesis} is a function $f: \X \rightarrow \Y$
that maps an instance $x\in \X$ to an outcome $y\in \Y$.
We work with a predetermined \emph{hypothesis class} $\F \subseteq \Y^\X$.

	\subsection{Statistical Definitions}
	Let us begin by  recalling a few well-studied notions from statistical learning theory. 

	\begin{definition}[VC Dimension, See \citep{shalev2014understanding}]
		Let $\X$ be an instance space and $\F$ be a hypothesis class on $\X$.
		$\F$ is said to shatter a set of points $S =\{ x_1, \dots ,x_m \} \subseteq \X$ if for each assignment of labels $y_1, \dots, y_m$ to $S$, there is a hypothesis $f \in \F$ such that for all $x_i \in S $, $f\left( x_i \right) =y_i$. 
		The VC dimension of $\F$ is  denoted by $\vcd \left( \F \right) $ and  is the largest cardinality of a set $S$ shattered by $\F$. 
	\end{definition}

    For any hypothesis class $\F$ on instance space $\X$, a learning algorithm $\A$ takes as input a sample set $S$ chosen i.i.d.\ from an underlying distribution $\D$ and returns a function that achieves near-optimal performance on $\D$.
    As we stated below, existence of algorithms that can learn a hypothesis class $\F$ is characterized by the VC dimension $\F$. 

	\begin{proposition}[See \citep{shalev2014understanding}] \label{fact:VC-sample}
Given a hypothesis class $\F$ on instance space $\X$,	there is a PAC learning algorithm $\A$ such that for any distribution $\D$ and any number of samples $m$,  with probability $1-\delta$ over $S\sim \D^m$, the function returned by the algorithm  $f_S = \A(S)$ satisfies
		\begin{equation} \Ex_{x\sim \D}\Bracks{f_{S}(x)} - \min_{f\in \F}~ \Ex_{x\sim \D}\Bracks{f(x)} \leq O\Parens{\sqrt{\frac{\vcd(\F)+ \ln(1/\delta)}{m}}}.   \label{eq:pac-bound}
		\end{equation}
		The above bound can be achieved by \emph{Empirical Risk Minimization} that uses $\A(S) = \argmin_{f\in \F}\Ex[f(x)]$. Furthermore, Equation~\eqref{eq:pac-bound} is known to be tight. That is, a hypothesis class is PAC learnable if and only if it has finite VC dimension.
		
		
	\end{proposition}
	We will use the notion of a cover of a hypothesis class, which is a set of functions $\F'$ that approximate every function in $\F$ under a given distribution. This is formally defined below.
	 
	\begin{definition}[$\beta$-cover]
		Let $\F$ be a hypothesis class. A set of function $\F'\subseteq \Y^\X$ is said to be a $\beta$-cover for $\F$ with respect to distribution $\D$ if for all $f \in \F$, there is a $f' \in \F'$ such that 
		\begin{equation*}
			\Pr_{x \sim  \D} \left[  f\left( x \right) \neq f'  \left( x \right)  \right] \leq \beta. 
		\end{equation*} 
	\end{definition}
	The following well-known fact bounds the size of a $\beta$-cover of any class  with respect to any distribution as a function of its VC dimension. 
			\begin{fact}[\cite{HAUSSLER1995217}] \label{fact:net_size}
				Let $\mathcal{F}$ be a hypothesis class with $d = \vcd(\F)$ and let $\D$ be any distribution over $\X$. 
				Then, $\F$ has a $\beta$-cover of size $ \left( \nicefrac{41}{\beta} \right)^d $ with respect to distribution $\D$.
			\end{fact}
	


	\subsection{Online Learning}

	\subsubsection{Standard Setting}
	
Online learning over a  hypothesis class $\F$ is a repeated game between a learner and an adversary over $T$ rounds.
	On round $t$, the learner chooses a distribution $q_t\in \Delta(\F)$
and then the adversary chooses an instance  $x_t \in \X$. After this, 
a function $f_t$ is realized from distribution $q_t$, the learner observes $x_t$, and suffers a loss of $f_t \left( x_t \right)$. 
	The objective of the learner is  to minimize the expected regret with respect  to the best fixed function $f\in \F$ in hindsight, defined as
	\begin{equation*}
	\regret_\F \left( \A \right) =   \Ex  \left[ \sum_{t =1 }^T f_t\left( x_t \right) - \min_{f \in \F }    \sum_{t =1 }^T f(x_t)  \right],
	\end{equation*} 
where the expectation is taken over the draws of $f_t\sim q_t$ for all $t\in [T]$. In this paper, we mainly consider \emph{adaptive adversaries}, where adversary's choice of $x_t$ can depend on the entire history of the game up to and including round $t-1$ and the knowledge of the algorithm.

The minmax regret is defined as the best possible regret that is achievable by any  algorithm against a worst case adaptive adversary.
	This can be written as 
	\begin{equation*}
		\regret_\F  =  \inf_{q_1} \sup _{x_{1} \in \X} \underset{ f_1 \sim q_1 }{\mathbb{E}}  \ldots \inf_{q_T}  \sup _{x_{T} \in \X}    \underset{ f_T \sim q_T }{\mathbb{E}}     \left[ \sum_{t =1 }^T f_t\left( x_t \right) - \min_{f \in \mathcal{H}  }    \sum_{t =1 }^T f(x_t)  \right].
	\end{equation*}
	 



Minmax regret can be used to bound the regret of variants of online learning. Below we give two such examples.
\begin{example}	
Consider the online prediction setting, where a learner has to predict labels of a sequence of points. 
That is, on round $t$ the adversary first picks an instance $x_t$ and present it to the learner. The learner then picks a distribution, the adversary picks a point $x_t$ and a label $y_t$ and then player samples a prediction $\hat{y}$. 
	The player suffers loss $ \mathbb{I} \left[ \hat{y}_t \neq y_t \right] $. 
	The objective of the player is to minimize his loss relative to the best fixed hypothesis in class $\mathcal{H}$ in hindsight. 
	Formally, regret of an algorithm $\mathcal{A} $ is defined as 
		\begin{equation*}
			\regret \left( \mathcal{A} \right) = \sum_{t =1 }^T \mathbb{I} \left[ \hat{y}_t \neq y_t \right] - \min_{h \in \mathcal{H}  }    \sum_{t =1 }^T \mathbb{I} \left[ h\left( x_t \right) \neq y_t \right]. 
		\end{equation*}
		The minmax regret is defined as minimum regret of an algorithm against a worst case adversary. 
		This can be written as 
		\begin{equation*}
			\regret \left( \mathcal{H} \right) =  \inf_{q_1} \sup _{x_{1} \in \mathcal{Z}} \underset{ \hat{y}_1 \sim q_1 }{\mathbb{E}}  \ldots \inf_{q_T}  \sup _{x_{T} \in \mathcal{Z}}    \underset{ \hat{y}_T \sim q_T }{\mathbb{E}}     \left[ \sum_{t =1 }^T \mathbb{I} \left[ \hat{y}_t \neq y_t \right] - \min_{h \in \mathcal{H}  }    \sum_{t =1 }^T \mathbb{I} \left[ h\left( x_t \right) \neq y_t \right]  \right]
		\end{equation*}
		where $q_i$ represents distributions over the predictions.
		Note that here the learner is not required to predict a hypothesis in class, and thus this is improper learning. 
		But note that the regret of an improper learning can be bounded by that of a proper learner and thus it is easy to see that the online prediction game can be captured using the earlier online learning model. 
\end{example}

	As with statistical learning, in the online setting, a combinatorial dimension captures the learnability. 
	This is known as the Littlestone dimension, which captures the largest depth of a mistake tree shattered by the class. 
	Formally, 

	\begin{definition}[Littlestone Dimension, See \citep{ben2009agnostic}]
		Let $\X$ be an instance space and $\F$ be a hypothesis class on $\X$. 
		A mistake tree is a full binary decision tree whose internal nodes are labelled by elements of $\X$. 
		For every choice of labels $ \{ y_i \}_{i=1}^d $, 
		Every root to leaf path in the mistake tree corresponds to a sequence $ \{  \left( x_i , y_i  \right) \}_{i=1}^{d}$ by associating a label $y_i$ to a node depending on whether it is the left or right child of its parent.   
		A mistake tree of depth $d$ is said to be shattered by a class $\F$ if for any root to leaf path $ \{  \left( x_i , y_i  \right) \}_{i=1}^{d}$, there is a function $f \in \F $ such that $ f\left( x_i \right) = y_i  $ for all $i \leq d$. 
		The Littlestone dimension of the class $\F$ denoted by $\lsd \left( \F \right) $ is the largest depth of a mistake tree shattered by the class $\F$. 
	\end{definition}



	The following analogue of \cref{fact:VC-sample} for online learning shows that the Littlestone dimension captures the regret of an optimal algorithm learning a hypothesis class. 
	In particular, it show that sublinear regret is achievable if and only if the Littlestone dimension is finite. 

	\begin{proposition}[\citep{ben2009agnostic}]
		Let $\X$ be an instance space and $\F$ be a hypothesis class on $\X$. 
		Then, there exists an online learning algorithm $\mathcal{A}$ such that 
		\begin{equation*}
			\regret \left( \mathcal{A} \right) \leq \sqrt{  \frac{1}{2}  \lsd \left( \F \right) T \log\left( T \right) }.
		\end{equation*}
		Furthermore, for any algorithm $\mathcal{A}'$, we have that
		\begin{equation*}
			\regret \left( \mathcal{A} '  \right) \geq \Omega \left(   \sqrt{  \lsd \left( \F \right) T  } \right) . 
		\end{equation*} 
	\end{proposition}

	\begin{figure}
		\centering
		\includegraphics{tree.pdf}
	\end{figure}
	


	In order to understand the definition of Littlestone dimension, it is instructive to consider the class of thresholds on the interval $ \left[ 0,1 \right]$,that is functions of the form $  h_{ \theta }  \left( x \right) = \mathbb{I} \left[  x \leq \theta   \right] $.  
	It is easy to see that the VC dimension of this class is $1$. 
	But it can be shown that the Littlestone dimension is unbounded.  
	To see this, construct a tree whose nodes at depth $i$ are indexed by $k 2^{-i}$.  
	Note that this tree is shattered by class $\F$ and can be extended to have arbitrary depth. 
	To see why this shattered tree gives a strategy for adversary to enforce linear regret, 
	This thus gives us an example of a hypothesis class which admits statistical learning but does not admit online learning.



	It is often easier to work directly with the loss instead of the hypothesis class. 
	In this notation, the minmax regret can be written as 
	\begin{equation*}
		\mathbf{Regret} \left( \F \right) =  \inf_{q_1} \sup _{x_{1} \in \X} \underset{ f_1 \sim q_1 }{\mathbb{E}}  \ldots \inf_{q_T}  \sup _{x_{T} \in \X}    \underset{ f_T \sim q_T }{\mathbb{E}}     \left[ \sum_{t =1 }^T f_t\left( x_t \right) - \min_{f \in \mathcal{H}  }    \sum_{t =1 }^T f(x_t)  \right].
	\end{equation*}





	\subsubsection{Smoothed Setting}

 In the main body of the paper, we will focus our attention to finite subsets usually $\left[ n \right]$.  


	In the smoothed online learning game, the actions of the adversary comprise of picking a sequence of $\sigma$-smooth distributions. 
	One can consider two models for the adversary in this model. 
	In the first model, which we refer to as the non-adaptive adversary the adversary decides this actions $\nadist_1 \dots \nadist_T$ in advance. 
	In this model, the actions of the adversary at time $t$ does not depend on the instantiations at previous times.  
	In the second and more relevant model, which we refer to as the adaptive adversary, the action of the adversary at time $t$ which is a smooth distribution $\adist_t$ is decided after seeing the instantiation of the past $x_1 \sim \adist_1 \dots x_{t-1} \sim \adist_{t-1} $.  
	As before, in this setting, the minmax regret can be written as 
		\begin{equation*}
			\mathbf{Regret} =  \inf_{q_1} \sup _{ \adist_1 } \Ex_{f_1 \sim q_1} \Ex_{x_1 \sim \adist_1}   \ldots \inf_{q_T} \sup _{ \adist_T } \Ex_{f_T \sim q_T} \Ex_{x_T \sim \adist_T} \left[ \sum_{t=1}^T f_t  \left( x_t  \right) - \inf_{f \in \F}   \sum_{t=1}^T f  \left( x_t  \right)  \right]. 
		\end{equation*}











	




	
	
	
